Data Efficient Evaluation of Large Language Models and Text-to-Image Models via Adaptive Sampling

Evaluating LLMs and text-to-image models is a computationally intensive task often overlooked. Efficient evaluation is crucial for understanding the diverse capabilities of these models and enabling comparisons across a growing number of new models and benchmarks. To address this, we introduce SubLIME, a data-efficient evaluation framework that employs adaptive sampling techniques, such as clustering and quality-based methods, to create representative subsets of benchmarks. Our approach ensures statistically aligned model rankings compared to full datasets, evidenced by high Pearson correlation coefficients. Empirical analysis across six NLP benchmarks reveals that: (1) quality-based sampling consistently achieves strong correlations (0.85 to 0.95) with full datasets at a 10\% sampling rate such as Quality SE and Quality CPD (2) clustering methods excel in specific benchmarks such as MMLU (3) no single method universally outperforms others across all metrics. Extending this framework, we leverage the HEIM leaderboard to cover 25 text-to-image models on 17 different benchmarks. SubLIME dynamically selects the optimal technique for each benchmark, significantly reducing evaluation costs while preserving ranking integrity and score distribution. Notably, a minimal sampling rate of 1% proves effective for benchmarks like MMLU. Additionally, we demonstrate that employing difficulty-based sampling to target more challenging benchmark segments enhances model differentiation with broader score distributions. We also combine semantic search, tool use, and GPT-4 review to identify redundancy across benchmarks within specific LLM categories, such as coding benchmarks. This allows us to further reduce the number of samples needed to maintain targeted rank preservation. Overall, SubLIME offers a versatile and cost-effective solution for the robust evaluation of LLMs and text-to-image models.

==> sections/dump.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-high_school_computer_science_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Highschool-Computer-Science}
    \label{fig:subject21}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-high_school_european_history_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Highschool-European-History}
    \label{fig:subject22}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-high_school_geography_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Highschool-Geography}
    \label{fig:subject23}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-high_school_government_and_politics_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Highschool-Government-and-Politics}
    \label{fig:subject24}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-high_school_macroeconomics_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Highschool-Macroeconomics}
    \label{fig:subject25}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-high_school_mathematics_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Highschool-Mathematics}
    \label{fig:subject26}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-high_school_microeconomics_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Highschool-Microeconomics}
    \label{fig:subject27}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-high_school_physics_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Highschool-Physics}
    \label{fig:subject28}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-high_school_psychology_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Highschool-{Psychology}}
    \label{fig:subject29}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-high_school_statistics_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Highschool-Statistics}
    \label{fig:subject30}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-high_school_us_history_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Highschool-US-History}
    \label{fig:subject31}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-high_school_world_history_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Highschool-World-History}
    \label{fig:subject32}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-human_aging_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Human-Aging}
    \label{fig:subject33}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-human_sexuality_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Human-Sexuality}
    \label{fig:subject34}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-international_law_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-International-Law}
    \label{fig:subject35}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-jurisprudence_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Jurisprudence}
    \label{fig:subject36}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-logical_fallacies_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Logical-Fallacies}
    \label{fig:subject37}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-machine_learning_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Machine-Learning}
    \label{fig:subject38}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-management_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Management}
    \label{fig:subject39}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-marketing_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Marketing}
    \label{fig:subject40}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-medical_genetics_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Medical-Genetics}
    \label{fig:subject41}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-miscellaneous_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Miscellaneous}
    \label{fig:subject42}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-moral_disputes_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Moral-Disputes}
    \label{fig:subject43}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-moral_scenarios_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Moral-Scenarios}
    \label{fig:subject44}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-nutrition_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Nutrition}
    \label{fig:subject45}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-philosophy_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Philosophy}
    \label{fig:subject46}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-prehistory_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Prehistory}
    \label{fig:subject47}
\end{figure}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-professional_accounting_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Professional-Accounting}
    \label{fig:subject48}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-professional_law_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Professional-Law}
    \label{fig:subject49}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-professional_medicine_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Professional-Professional-Medicine}
    \label{fig:subject50}
\end{figure}

\begin{figure}[htbp]
\centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-professional_psychology_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Professional-Psychology}
    \label{fig:subject51}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-public_relations_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Public-Relations}
    \label{fig:subject52}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-security_studies_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Security-Studies}
    \label{fig:subject53}
\end{figure}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-sociology_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Sociology}
    \label{fig:subject54}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-us_foreign_policy_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-US-Foreign-Policy}
    \label{fig:subject55}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-virology_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-Virology}
    \label{fig:subject56}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/xlim_hendrycksTest-world_religions_50model_20modelsamplinginterval_0.21initialpct_0.01pctincrement.JPG}
    \caption{Data Sampling in Top 50 models of HendrycksTest-World-Religions}
    \label{fig:subject57}
\end{figure}


\begin{comment}
\textbf{Experiment Design}: 
\begin{enumerate}
    \item We utilize the model results provided by the Open LLM Leaderboard \cite{huggingface_openllm} across multiple benchmarks. Based on these results, we select the Top 50 models from each benchmark with a sampling interval of 20.
    \item We apply three different sampling techniques: quality-based sampling, random sampling, and clustering-based sampling, with sampling percentage ranges from 1\% to 100\% for each technique. 
    \item We plot the rank preservation coefficient against the sampling percentage for each benchmark and sampling technique, to analyse which sampling method performs ideally for which benchmark.
    \item We use the rank preservation coefficient as the primary evaluation metric to assess the quality of sampled subsets. Additionally, we consider variance analysis to understand the variability in sampling distribution across benchmarks.
    \item We identify the best sampling method for each benchmark based on the rank preservation coefficient and variance analysis. The goal is to recommend the sampling approach that best suits the characteristics of each dataset.
    \item We dynamically select the sampling techniques that perform optimally at a 10\% sampling percentage. This allows us to selectively sample the top 10\% subset, which generalizes well across the dataset, reducing computational overhead by 1/10 times.
\end{enumerate}
\end{comment}
